Embodied BERT: A Transformer Model for Embodied, Language-guided Visual Task Completion

Language-guided robots performing home and office tasks must navigate in and interact with the world. Grounding language instructions against visual observations and actions to take in an environment is an open challenge. We present Embodied BERT (EmBERT), a transformer-based model which can attend to high-dimensional, multi-modal inputs across long temporal horizons for language-conditioned task completion. Additionally, we bridge the gap between successful object-centric navigation models used for non-interactive agents and the language-guided visual task completion benchmark, ALFRED, by introducing object navigation targets for EmBERT training. We achieve competitive performance on the ALFRED benchmark, and EmBERT marks the first transformer-based model to successfully handle the long-horizon, dense, multi-modal histories of ALFRED, and the first ALFRED model to utilize object-centric navigation targets.

==> 98_checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section X.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} % \JTi{To be filled when the paper is finished and each author has made a pass.} \ASi{Yes}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{sec:limitations}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{We are working towards public release of the modeling code to accompany the camera-ready version of the paper.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Sections~\ref{sec:model} and \ref{sec:results} and the Appendix.} % \JTi{Revisit if we end up not having Appendix details.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Training \modelac\ on the ALFRED benchmark takes a day or more for validation results, and multiple leaderboard submissions for test set results are not allowed to avoid models over-fitting the test set.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Details can be found in Section~\ref{par:impl_details}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, we have cited the ALFRED benchmark~\cite{alfred} and its backend simulator, AI2THOR~\cite{ai2thor}.}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{We discuss briefly the creation of the ALFRED benchmark in Section~\ref{sec:task}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{We leave this discussion to the ALFRED benchmark~\cite{alfred}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{We use existing resources from the ALFRED benchmark and do not collect additional data.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> tables/all_results.tex <==
\begin{table*}
    \setlength{\aboverulesep}{0pt}
    \setlength{\belowrulesep}{0pt}
    \centering
    \begin{small}
    \begin{tabular}{@{}c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 4pt}c@{\hskip 4pt}crrrr@{}}
                     & & & & & & \mcp{4}{\textbf{Validation Fold Performance}} \\
                     \mcc{6}{\basemodels{\modelac}} & \mcc{2}{\splits{Seen}}   & \mcc{2}{\splits{Unseen}}  \\
                     Init Weights & \#SB & Mem & Nav $O$ & $P(O)$ & VRC & \multicolumn{1}{c}{Task} & \multicolumn{1}{c}{GC} &
                     \multicolumn{1}{c}{Task} & \multicolumn{1}{c}{GC} \\
    \toprule
    \addlinespace[-\aboverulesep]
    \midrule
    OSCAR & 18 & 200 & \cblkmark & \cblkmark & \cblkmark & 28.54 (22.88) & 38.69 (31.28) & \phantom{0}1.46 (\phantom{00}.72) & 10.19 (\phantom{0}6.25) \\[1pt]
    OSCAR & 18 & 200 & \cblkmark & & \cblkmark & 34.76 (28.46) & 41.30 (35.50) & \phantom{0}3.66 (\phantom{0}1.55) & 12.61 (\phantom{0}7.49) \\[1pt]
    OSCAR & 18 & 200 & \cblkmark & \cblkmark & & 36.22 (27.05) & 44.57 (35.23) & \phantom{0}4.39 (\phantom{0}2.21) & 13.03 (\phantom{0}7.54) \\[1pt]
    OSCAR & 18 & 200 & \cblkmark & & & \B{37.44} (\B{28.81}) & \B{44.62} (\B{36.41}) & \B{\phantom{0}5.73} (\B{\phantom{0}3.09}) & \B{15.91} (\B{\phantom{0}9.33}) \\[1pt]
    OSCAR & 18 & 200 & & & & 23.66 (17.62) & 29.97 (24.16) & \phantom{0}2.31 (\phantom{0}1.24) & 12.08 (\phantom{0}7.62) \\[1pt]
    BERT & 18 & 200 & \cblkmark & \cblkmark & &  26.46 (19.41)   &  35.70 (27.04)    & \phantom{0}3.53 (\phantom{0}1.77)   & 13.02 (\phantom{0}7.57)  \\[1pt]
    \midrule
    OSCAR & 9 & 200 & \cblkmark & \cblkmark & \cblkmark & 29.30 (20.14)   &  36.28 (27.21)    & \phantom{0}3.06 (\phantom{0}1.13)   & 12.17 (\phantom{0}6.69) \\[1pt]
    OSCAR & 9 & 200 & \cblkmark & \cblkmark & & 31.75 (23.52)   &  38.80 (32.21)    & \phantom{0}2.56 (\phantom{0}1.28)   & 12.97 (\phantom{0}8.24)  \\[1pt]
    OSCAR & 9 & 200 & & \cblkmark & \cblkmark & 20.37 (16.30)   &  28.64 (23.11)    & 1.46 (\phantom{0}0.75)   & 10.47 (\phantom{0}6.26)  \\[1pt]
     OSCAR & 9 & 200 & \cblkmark & & \cblkmark & 29.02 (21.40)   &  36.27 (28.37)    & \phantom{0}2.68 (\phantom{0}1.42)   & 11.04 (\phantom{0}6.33)  \\[1pt]
    OSCAR & 9 & 200 & \cblkmark & &  & 28.33 (20.77)   &  36.83 (28.03)    & \phantom{0}2.68 (\phantom{0}1.18)   & 11.60 (\phantom{0}6.78)  \\[1pt]
    OSCAR & 9 & 200 & & & & 27.84 (20.66)   &  36.59 (27.97)    & \phantom{0}2.44 (\phantom{0}1.06)   & 11.46 (\phantom{0}6.76)  \\[1pt]
    % \midrule
    % 9 & 200 & \cblkmark & \cblkmark & MSV &  28.27 (19.32)   &  36.98 (28.11)    & \phantom{0}3.66 (\phantom{0}1.66)   & 12.99 (\phantom{0}6.82)  \\[1pt]
    % 9 & 200 & \cblkmark & \cblkmark & BERT &  27.68 (19.35)   &  36.46 (28.00)    & \phantom{0}4.15 (\phantom{0}1.92)   & 13.56 (\phantom{0}7.12)  \\[1pt]
    \midrule
    OSCAR & 0 & 200 & \cblkmark & \cblkmark & &  25.31 (18.79)   &  34.27 (26.09)    & \phantom{0}3.42 (\phantom{0}1.49)   & 12.25 (\phantom{0}7.34)  \\[1pt]
    OSCAR & 9 & 1 & \cblkmark & \cblkmark & & 20.98 (13.98)   &  33.33 (22.74)    & \phantom{0}1.10 (\phantom{0}0.60)   & 10.33 (\phantom{0}4.69)  \\[1pt]
    OSCAR & 18 & 1 & \cblkmark & \cblkmark & & 21.95 (12.99) & 35.04 (22.31) & \phantom{0}1.58 (\phantom{00}.54) & 11.08 (\phantom{0}6.18) \\[1pt]
    \addlinespace[-\belowrulesep] 
    \bottomrule
    \mcc{6}{\basemodels{MOCA}~\cite{moca}} & 18.90 (13.20)   &  28.02 (21.81)    & \phantom{0}3.65 (\phantom{0}1.94)   & 13.63 (\phantom{0}8.50) \\[1pt]

    \bottomrule
    \end{tabular}
    \caption{\textbf{Validation Fold Performance.}
    We present ablations adjusting the number of side-view bounding boxes, attended memory length, with and without predicting navigation target $O$, target parent object $P(O)$, and visual region classification (VRC) loss. 
    We also explore initializing our multi-modal encoder with BERT versus OSCAR initialization.
    The highest values per fold and metric are \textbf{bolded}.
    }
    \label{tab:all_ablations}
    \end{small}
\end{table*}

==> tables/subgoal_results.tex <==
\begin{table}
\centering
\begin{small}
% \begin{tabular}{@{}l@{\hspace{8pt}}acac@{}}
%            & \multicolumn{4}{c}{Sub-Goal Ablations - \textbf{Validation}} \\
%            & \mcc{2}{\basemodels{\modelac}} & \mcc{2}{\basemodels{MOCA}~\cite{moca}}    \\
% Sub-Goal   & \splits{Seen} & \splits{Unseen} & \splits{Seen} & \splits{Unseen} \\
% \toprule
% Goto       & \B{\phantom{0}56} & \phantom{0}23 & 54 & \B{32} \\ 
% Pickup     & \B{\phantom{0}78} & \B{\phantom{0}74} & 53 & 54 \\ 
% Put        & \B{\phantom{0}82} & \B{\phantom{0}54} & 62 & 39 \\ 
% Cool       & \B{\phantom{0}96} & \B{100} & 87 & 38 \\  
% Heat       & \B{100} & \B{\phantom{0}95} & 84 & 86 \\ 
% Clean      & \B{\phantom{0}90} & \B{\phantom{0}81} & 79 & 71 \\ 
% Slice      & \B{\phantom{0}85} & \B{\phantom{0}71} & 51 & 55 \\ 
% Toggle     & \B{100} & \B{\phantom{0}51} & 93 & 11 \\  
% \midrule                             
% Average    & 85.81 & 68.44 & 70.37 & 48.25 \\ 
% \bottomrule
% \end{tabular}
% \hfill\
\begin{tabular}{@{}l@{\hspace{8pt}}acac@{}}
           & \multicolumn{4}{c}{Task Type Performance - \textbf{Validation}} \\
           & \mcc{2}{\basemodels{\modelac}} & \mcc{2}{\basemodels{MOCA}~\cite{moca}}    \\
Sub-Goal   & \splits{Seen} & \splits{Unseen} & \splits{Seen} & \splits{Unseen} \\
\toprule
\task{pick}       & 29.32 & 1.00 & \B{29.50} & \B{\phantom{0}5.00} \\ 
\task{stack}      & \B{6.86} & \B{1.83} & 5.20 & \phantom{0}1.80 \\ 
\task{pick two}   & 9.17 & 0.00 & \B{11.20} & \B{\phantom{0}1.10} \\ 
\task{clean}      & \B{28.04} & \B{5.31} & 22.30 & \phantom{0}2.40 \\  
\task{heat}       & \B{21.78} & 0.00 & 15.80 & \B{\phantom{0}2.70} \\ 
\task{cool}       & \B{33.61} & 0.00 & 26.10 & \B{\phantom{0}0.70} \\ 
\task{examine}    & \B{28.72} & 1.16 & 20.20 & \B{13.20} \\ 
%& & & & \\ 
% \midrule                             
% Average    & 22.50 & 1.33 & 18.61 & 3.84 \\
\bottomrule
\end{tabular}
\end{small}
\caption{% \textbf{Sub-goal (left) and task type (right) success rates.}
\textbf{Success rates by task type.}
% Sub-goal success is calculated by following the oracle trajectory until the sub-goal of interest, then requiring the agent to perform inference only during that sub-goal, with success calculated locally against the goal.
% For example, if the agent is able to \texttt{Goto} the correct destination after being guided in previous sub-goals by the oracle trajectory, that sub-goal is marked as success.
Task type success is the validation success (Table~\ref{tab:ablation_results}) rate broken down by ALFRED task type.
The highest values per fold and task are shown in \B{blue}.
}
\label{tab:subtask_ablations}
\end{table}

